Self-Sampling Meta SAM: Enhancing Few-shot Medical Image Segmentation with Meta-Learning

While the Segment Anything Model (SAM) excels in semantic segmentation for general-purpose images, its performance significantly deteriorates when applied to medical images, primarily attributable to insufficient representation of medical images in its training dataset. Nonetheless, gathering comprehensive datasets and training models that are universally applicable is particularly challenging due to the long-tail problem common in medical images. To address this gap, here we present a Self-Sampling Meta SAM (SSM-SAM) framework for few-shot medical image segmentation. Our innovation lies in the design of three key modules: 1) An online fast gradient descent optimizer, further optimized by a meta-learner, which ensures swift and robust adaptation to new tasks. 2) A Self-Sampling module designed to provide well-aligned visual prompts for improved attention allocation; and 3) A robust attention-based decoder specifically designed for medical few-shot learning to capture relationship between different slices. Extensive experiments on a popular abdominal CT dataset and an MRI dataset demonstrate that the proposed method achieves significant improvements over state-of-the-art methods in few-shot segmentation, with an average improvements of 10.21% and 1.80% in terms of DSC, respectively. In conclusion, we present a novel approach for rapid online adaptation in interactive image segmentation, adapting to a new organ in just 0.83 minutes. Code is publicly available on GitHub upon acceptance.

==> 1_Abstract.tex <==
\begin{abstract}
While the Segment Anything Model (SAM) excels in semantic segmentation for general-purpose images, its performance significantly deteriorates when applied to medical images, primarily attributable to insufficient representation of medical images in its training dataset. Nonetheless, gathering comprehensive datasets and training models that are universally applicable is particularly challenging due to the long-tail problem common in medical images.
%While the Segment Anything Model (SAM) performs better semantic segmentation for everyday images, its proficiency falters in areas like medical images, largely due to the absence of such scenarios in its training material. 
%However, collecting all representative datasets and training a universal model for each industry is arguably impossible, especially for the long-tail distribution of medical images. 
%f
To address this gap, here we present a \textbf{\underline{S}elf-\underline{S}ampling \underline{M}eta \underline{SAM}} (SSM-SAM) framework for few-shot medical image segmentation. Our innovation lies in the design of three key modules: 1) An online fast gradient descent optimizer, further optimized by a meta-learner, which ensures swift and robust adaptation to new tasks. %, enhancing its robustness; 
%1) A fast online gradient descent meta-learner, empowering the model to swiftly transfer and adapt to new tasks.
2) A Self-Sampling module designed to provide well-aligned visual prompts for improved attention allocation; and 3) A robust attention-based decoder specifically designed for few-shot medical image segmentation to capture relationship between different slices.
%
%Our meta-learner enables the model to transfer and adapt to new tasks with enhanced robustness swiftly. 
%Extensive experiments on two different medical image datasets, abdomen CT and abdomen MRI, demonstrate the superiority of our framework over existing state-of-the-art methods. 
Extensive experiments on a popular abdominal CT dataset and an MRI dataset demonstrate that the proposed method achieves significant improvements over state-of-the-art methods in few-shot segmentation, with an average improvements of 10.21\% and 1.80\% in terms of DSC, respectively. 
In conclusion, we present a novel approach for rapid online adaptation in interactive image segmentation, 
%
adapting to a new organ in just 0.83 minutes. Code is publicly available on GitHub upon acceptance. %\href{https://github.com/ZHymLumine/SAM_Adapter}{this https URL} 
\end{abstract}


==> 2_Introduction.tex <==
\section{Introduction}
% Semantic segmentation plays a pivotal role in image analysis by delineating objects within images, driving advancements in fields ranging from medical diagnostics to autonomous vehicles. The Segment Anything Model (SAM) \cite{kirillov2023segment} has emerged as a beacon in this domain, exhibiting commendable performance in everyday image scenarios. However, as with many models, its prowess seems to waver when confronted with nuanced tasks such as shadow segmentation, medical image, and the detection of transparent objects \cite{ji2023segment}, which are also of paramount importance in the fields of autonomous driving, medical applications, and industrial production. One reason for this limitation can be attributed to the absence of such scenes in SAM's training data.

Medical image segmentation plays a pivotal role in clinical applications, including disease diagnosis, abnormality detection and treatment planning. Historically, the segmentation of anatomical structures was performed manually by experienced physicians, a laborious and time-consuming task.
%Medical image segmentation is crucial for clinical applications like disease diagnosis and treatment planning. Traditionally, experienced doctors manually segmented anatomical structures, which is a time-consuming process.
%
Recent advancements in deep learning offer automated segmentation tools that deliver near-human accuracy swiftly. Nevertheless, these tools need extensive training on large annotated datasets for optimal performance, which are costly and time-intensive since they require inputs from experts with extensive clinical experience. Thus, in the field of medical imaging, few-shot learning \cite{snell2017prototypical, li2021adaptive, zhang2021self} has gained significant interest from researchers because it is able to segment accurately without extensive labeled data. In fact, to achieve optimal performance on unseen classes, few-shot learning models must excel in extracting representative features from limited data. However, current few-shot learning frameworks for medical image segmentation \cite{dong2018few, wang2019panet, tang2021recurrent} predominantly pretrain their models using data from a single medical domain, often with restricted datasets, leading to limited feature extraction ability. If we can leverage the strong feature extraction ablities obtained from extensive training data of diverse domains, the model can capture more distinctive features, enhancing its adaptability to new tasks. 
% -
%However, to achieve excellent performance in the unseen classes, the pretrained model in few-shot learning is required to extract representative features from the limited data. Current few-shot learning frameworks for medical image segmentation only pretrain their model with data from a single domain with limited data. An extensive amount of data across different domainss may help the model capture more distinctive features which benefit adapting to new tasks.  
% -

Recently, Segment anything model (SAM) \cite{kirillov2023segment} has attracted significant attention. Trained on a large segmentation dataset of over 1 billion masks across various domains of natural images, SAM has strong feature extraction and generalization abilities and can segment any object on a certain image. Given SAM's excellent zero-shot transferability, a natural idea is to directly apply SAM for medical image segmentation to address the issue of relatively scarce medical image data \cite{roy2023sam, he2023accuracy}. However, recent studies \cite{mazurowski2023segment, shi2023generalist} have shown that the performance of SAM is overall moderate and varies significantly across different datasets and different cases, demonstrating the potential promise of SAM within the context of medical images but also shows that the model cannot be applied directly  with high confidence. %significantly drops when dealing with medical images. 
Such phenomenon is attributed to the vast differences between natural and medical images, as SAM was primarily trained on natural images.
To better adapt SAM to medical images, most prior studies focused on integrating lightweight Adapters \cite{chen2023sam, wu2023medical} or on freezing the heavy image and prompt encoders, opting to fine-tune solely the mask decoder \cite{ma2023segment, hu2023skinsam, li2023polyp}. However, the limited data available for unseen classes will hinder the few-shot segmentation performance of these approaches.
% Nevertheless, due to the long-tail distribution of medical images and the fact that annotating these images requires specialized knowledge and a significant amount of time, obtaining a comprehensive collection of medical images is not practical. 

Driven by the desire to maximize the powerful extracted features of SAM through prompts \cite{zhang2023survey}, and to leverage its potential zero-shot capabilities without vast training data, we introduce the Self-Sampling Meta SAM (SSM-SAM) framework, which utilizes a Meta-learning method MAML++. Our framework consists of two main parts. The first part is a redesigned backbone that removes the original SAM's prompt encoder and mask decoder; instead, we employ a self-sampling prompt encoder and Flexible Mask Attention Decoder (FMAD). Also, we integrate adapters into the image encoder as previous works do, allowing SAM to learn features of unfamiliar tasks. This enables SAM to have better transferability for few-shot learning and is termed \textbf{SS-SAM} (\underline{S}elf-\underline{S}ampling \underline{SAM} without MAML++). The second part, which we refer to as \textbf{SSM-SAM} (with MAML++), serves as our final framework for few-shot learning. It is a meta-learning based optimizer layered on top of this backbone to further boost SAM's few-shot performance on medical images.
 
We performed experiments for few-shot learning on an abdomen CT dataset and an MRI dataset. We also utilized a fully supervised medical image segmentation task to evaluate the performance of our SS-SAM backbone (without MAML++) in comparison to prior methods on CT dataset. 

Our contributions are summarized as follows:
\begin{itemize}
    \item An effective online parameter adaptation technique  optimized by a MAML++ \cite{antoniou2018train} based meta-learner to enhance SAM's generalization and few-shot learning capacities. 
    %This plug-and-play approach allows for easy transfer to new foundation models without extensive effort.
    \item A positive-negative self-sampling module that can generate aligned visual prompts to better extract the contextual relationship.
    % \item A replacement of mask decoder with iterative convolution and upsampling decoder, illustrated in Fig \ref{fig:3}, which optimizes the model's segmentation acuity without adding undue computational weight.
    \item A novel Flexible Mask Attention Decoder specifically designed for medical image few-shot segmentation.
    % \item For the first time, we introduce a universal approach to optimize and transfer visual foundational models to unfamiliar tasks. Every module we employ is plug-and-play, ensuring effortless transferability to new foundation models without compromising performance.
    \item Our method outperformed the SOTA framework for few-shot medical image segmentation by an average of 10.21\% on MICCAI15 Multi-Atlas Abdomen Labeling challenge dataset \cite{MICCAI} and 1.80\% on ISBI 2019 Combined Healthy Abdominal Organ Segmentation Challenge \cite{kavur2021chaos} in terms of DSC.
    % \item Experimental results demonstrate the effectiveness and superiority of the proposed SSM-SAM compared to the previous competing methods on both fully supervised and few-shot medical image segmentation.
\end{itemize}

Each module we use is plug-and-play, aiming to facilitate the deployment of fast and robust online image segmentation systems across various industries and making our model a baseline for improving performance where foundational models like SAM have struggled in the past.

% First, to validate the effectiveness of our backbone framework in comparison to prior methods, we utilize a fully supervised medical image segmentation task to assess the performance of our SS-SAM backbone.
% Then, considering the common long-tail disparities in medical images, we mainly focus on few-shot medical image segmentation as a representative task to underscore the substantial advantages provided by SSM-SAM since it is time-consuming and knowledge-required to annotate such a large amount of medical data in real-world scenarios \cite{milletari2016v, deselaers2008automatic, budd2021survey, ko2012automatic, lutnick2019integrated}.

==> 3_RelatedWork.tex <==
\section{Related Work}
\begin{figure*}[ht]
\centering
\includegraphics[height=5.1cm]{fig/architecture.pdf}
\caption{Overview of our proposed framework for SSM-SAM. SSM-SAM backbone consists of three main components:
a) Injecting Adapters into the encoder of SAM to quickly acquire task-related information.
b) Using the Self-Sampling Module to replace the position encoding based prompt encoder to strengthen the relationship between the feature and the prompt.
c) Flexible Mask Attention Decoder (FMAD) to enhance boundary information and refine the final generated mask map. On top of the backbone, we employ a meta-learning based online optimizer.}
\label{fig:1}
\end{figure*}

\noindent\textbf{Foundation Models.} A foundation model is essentially a large pre-trained model, typically developed using self-supervised learning across diverse datasets. This allows it to be fast adapted to specific tasks through mechanisms by fine-tuning or in-context learning. At present, foundation models have reached a level of maturity in the NLP domain, with models like BERT \cite{devlin2018bert}, GPT-3 \cite{brown2020language}. 
 In the realm of computer vision, the Segment Anything Model (SAM) \cite{kirillov2023segment}, pre-trained on 11M images with 1B masks, first introduced a foundation model for image segmentation. This model can interpret a variety of prompts given by users, such as points, boxes, masks, and texts, to generate user-specified segmentations and is adept at segmenting any object within an image. However, despite its zero-shot generalization capabilities, SAM has demonstrated sub-optimal performance across multiple downstream tasks \cite{ji2023segment}. This observation has stimulated ongoing research efforts to enhance SAM's performance in these tasks \cite{ma2023segment, wu2023medical, gong20233dsamadapter, zhou2023sam}. \\
\noindent\textbf{Adapters.} 
Adapters have emerged as a powerful tool in the realm of transfer learning for NLP and computer vision. Introduced as a lightweight alternative to full model fine-tuning, adapters allow for model customization while preserving the pre-trained parameters \cite{houlsby2019parameter}. Instead of updating all the parameters in the model, adapter methods insert small bottleneck layers in the model architecture, which are then fine-tuned while the original model parameters remain unchanged. Recently, the ViT-Adapter \cite{chen2022vision} has been developed to equip a standard ViT \cite{dosovitskiy2021image} with the capability to perform a variety of downstream tasks. In a further development, an Explicit Visual Prompting (EVP) \cite{liu2023explicit} technique has facilitated the integration of explicit visual cues into the Adapters. In this work,  We integrate such Adapters \cite{chen2023sam} into the image encoder of SAM to avoid training a large amount of parameters. \\
\noindent\textbf{Visual Prompts.} 
The application of visual prompts in computer vision tasks has its roots in interactive segmentation, a methodology that necessitates user input, such as clicks \cite{xu2016deep, wang2018interactive, jang2019interactive, lin2020interactive, chen2021conditional}, bounding boxes \cite{wu2014milcut, rajchl2016deepcut}, or scribbles \cite{batra2010icoseg, bai2014error, lin2016scribblesup}, or convert spatial queries to masks and feed them into the image backbone \cite{liu2022simpleclick} to assist the algorithm in accurately delineating object boundaries. These visual prompts augment the segmentation process, yielding more accurate and dependable outcomes \cite{wang2023review}. 
However, such form of visual prompts either struggle to adapt to unseen prompts \cite{kirillov2023segment} or might be heavy in applications as each interaction necessitates processing the image through the feature extractor \cite{liu2022simpleclick}. Recently, visual sampler has been introduced to transform all non-textual queries into visual prompts that reside within the same visual embedding space to address these limitations \cite{zou2023segment}. However, no prior research has endeavored to employ this approach for generating prompts using the SAM trained on an extensive image corpus. Here we seek to bridge this research gap. \\
\noindent\textbf{Model Agnostic Meta Learning (MAML).} One continuous challenge of few-shot medical image segmentation is the distribution mismatch between training and testing datasets, particularly the long tail problem. 
Fortunately, MAML \cite{finn2017model} and MAML++ \cite{antoniou2018train} offers meta-learning frameworks tailored to combat this issue. It is elegantly simple yet can find suitable model-agnostic initialization parameters that are trained through various tasks and can quickly adapt to new tasks. Many previous works like\cite{makarevich2021metamedseg,singh2021metamed,yu2020foal} use meta-learning to address different problems in medical image segmentation. Yet, MAML++ framework has been primarily focused on vision tasks like classification and recognition. All these previous works inspired us to utilize MAML++ to enhance foundational models' few-shot learning ability.




% \noindent\textbf{Shadow Detection?} aims to quantify the reliability of a result $e.g.,$ a confidence distribution of each class rather than a certain angle value for pose data \cite{prokudin2018deep}. A well-calibrated uncertainty is especially important for large systems to assess the consequence of a decision \cite{che2019deep,han2019unsupervised}. \cite{prokudin2018deep} proposes to output numerous sets of the mean and variation of Gaussian/Von-Mises distribution following \cite{beyer2015biternion}. It is unnecessarily complicated and is a somewhat ill-matched formulation as it assumes the pose label is continuous, while it is discrete. We argue that the $softmax$ is a natural function to capture discrete uncertainty, and is compatible with Wasserstein training.



==> 4_Approach.tex <==
\section{Methodology}
\subsection{Overview of SSM-SAM architecture}
%SAM consists of three core components: an image encoder, a flexible prompt encoder, and a lightweight mask decoder. 
\cref{fig:1} depicts the architecture of our few-shot learning framework.
We keep the image encoder of SAM frozen and add a learnable \textbf{Adapter} layer \cite{liu2023explicit} to each of the transformer layers for parameter-efficient training. After passing through the image encoder, we perform a self-sampling operation on the first image embedding to update it. Afterward, we feed the four output image embeddings into our Flexible Mask Attention Decoder (FMAD) %to refine these features and apply a series of convolution and upsampling 
to refine these embeddings and generate the predicted mask. On top of this backbone, we implement a MAML++ based meta-learner to search for optimal initialization parameters for rapid adaptation to different organs. %Note that for evaluating our backbone in a fully supervised setting, we remove the attention-based module and directly upsample these features to produce the mask.% The architecture is depicted in \cref{fig:1}.
% SAM consists of three core components: an image encoder, a flexible prompt encoder, and a lightweight mask decoder. The image encoder of SAM uses a Vision Transformer (ViT) \cite{dosovitskiy2021image}, which is pre-trained with MAE \cite{he2022masked}. When given an image of any size, it is essential to first resize it to a resolution of 1024 x 1024. The ViT then processes this resized image to generate an image embedding with dimensions $C\times H\times W$. For this research, we chose the ViT-B variant (SAM-b), (where $C$ = 256, $H$ = 64, $W$ = 64). To avoid fine-tuning the whole large image encoder of SAM, we keep it frozen and add an learnable \textbf{Adapter} layer \cite{liu2023explicit} to each of the 12 transformer layers in the image encoder. We only train the parameters within \textbf{Adapters}, which are tasked with learning task-specific knowledge and low-level structural information from the features extracted from image embeddings. For the $k$-$th$ Adapter layer , we take patch embedding $\text{F}^{k}$ as input and obtain updated parameters $\text{P}^{k}$
% \begin{equation} 
% \text{P}^{k} = \text{{MLP}}_{\text{{up}}}(\text{{GELU}}(\text{{MLP}}^{k}_{\text{{tune}}} (F^{k}))
% \end{equation}
% where $\text{{MLP}}^{k}_{\text{{tune}}}$ refers to a linear layer within each Adapter for generating distinct prompts. $\text{{MLP}}_{\text{{up}}}$ is an up-projection layer shared across all Adapters designed to match the dimension of transformer features. $\text{P}^{k}$ represents the output  associated with each transformer layer. 

% Also, we divided image encoder to four sub-blocks, which is carried out with the intent of deriving multi-level information \cite{li2022exploring}. After passing through the image encoder, there are four embeddings of size $B \times C \times H \times W $. We perform a self-sampling operation on the first image embedding to update it. Subsequently, these four features are individually input into the Flexible Mask Attention Module (FMAM) to form a feature of size $B \times 1024 \times 64 \times 64$. We then apply a series of convolution and upsampling to generate the predicted mask. Note that for fully supervised learning, we only remove the Flexible Mask Attention Module in the decoder, and all other parts remain the same. We use an online meta-learning-based optimizer for few-shot learning to fast adapt to unseen organs. 


 
% To avoid training the whole large image encoder of SAM, we keep it frozen and introduce a minimal amount of learnable parameters \cite{liu2023explicit}. We only train these parameters within \textbf{Adapter} layers are tasked with learning task-specific knowledge and low-level structural information from the features extracted from image embeddings. For the $k$-$th$ layer Adapter, we take patch embedding $\text{F}^{k}$ as input and obtain updated parameters $\text{P}^{k}$
% \begin{equation} 
% \text{P}^{k} = \text{{MLP}}_{\text{{up}}}(\text{{GELU}}(\text{{MLP}}^{k}_{\text{{tune}}} (F^{k}))
% \end{equation}
% where $\text{{MLP}}^{k}_{\text{{tune}}}$ refers to a linear layer within each Adapter for generating distinct prompts. $\text{{MLP}}_{\text{{up}}}$ is an up-projection layer shared across all Adapters designed to match the dimension of transformer features. $\text{P}^{k}$ represents the output  associated with each transformer layer.

% SAM consists of three primary components: an image encoder, a prompt encoder, and a mask decoder. The image encoder, rooted in a pre-trained Vision Transformer (ViT) using Masked AutoEncoder (MAE), utilizes the ViT-H/16 variant, characterized by 14×14 windowed attention and four evenly distributed global attention blocks. This results in a 16× downsampled embedding of the input image. The prompt encoder can process either sparse inputs (such as points, boxes, or text) or dense ones (like masks). The mask decoder is a Transformer decoder block, adapted to include a dynamic mask prediction head. SAM employs bidirectional cross-attention, utilizing prompt-to-image and image-to-prompt embedding in each block to facilitate learning the interplay between the prompt and image embeddings. After executing two blocks, SAM increases the resolution of the image embedding, and a MLP maps the output token to a dynamic linear classifier, predicting the target mask for the provided image. In this study, we exclusively focus on the ViT-B/16 variant, which maintains only one-seventh of the parameters of ViT-H/16. This choice is intended to highlight the efficiency of our model, even with a substantially reduced parameter count.




 

==> 4_Approach1.tex <==
\subsection{Few-shot Online Optimizer}
Segmentation models' clinical deployment has historically been hindered by a distribution mismatch between training and testing datasets. Given the impossibility of collecting comprehensive representative data, we have innovated in our training approach. Rather than creating a universal offline model, we designed our model to recognize and adapt to new data types, ensuring it remains relevant for unseen images. In our few-shot medical image segmentation scenario, we consider a distribution over organs, denoted as $p(O)$, to which we aim our model to adapt. We represent our model as $f_\theta$ with parameter $\theta$, which is trained on images of different organs, $I_{o_i}$, following the distribution $p(I_{o_i})$, where $o_i$ signifies the $i^{th}$ organ. The online optimizer optimizes the parameters via back-propagating steps as follows:
\begin{equation}
    \theta_i^{'} \leftarrow \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{o_i}(f_{\theta_i^{'}})
\end{equation}
where $\alpha$ is the learning rate and $\theta_i^{'}$ represents the model parameters adapted to fit the $i^{th}$ organ. We employ balanced cross-entropy and IoU loss to supervise our network so $L_{o_i}$ can be expressed as: 
\begin{equation}
\label{loss}
    L_{o_i} = L_{bce} + L_{iou}
\end{equation}
The overview of the online optimizer is outlined in \cref{online}.

\begin{algorithm}
\caption{SSM-SAM Online Optimizer}
\label{online}
\begin{algorithmic}[1] % '1' 表示每行都显示数字
\IState \textbf{Input:} $K$ image-mask pairs $P_{i}=\{(I_{i},M_{i})_k\}$ of the target organ $o_i$
\IState \textbf{Input:} trained parameters: $\theta$
\IState \textbf{Require:} learning rate $\alpha$; number of online optimization steps $S$
\State $\theta_i^{'} \gets \theta$
\For{$s$ from 1 to $S$}
    \For{$(I_i,M_i)_k$ in $P_i$}
        \State Update parameters with gradient descent:
        \Statex \hspace{3em} $\theta_i^{'} \gets \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{O_i}(f_{\theta_i^{'}}((I_i,M_i)_k))$
    \EndFor
\EndFor
\IState \textbf{Output:} updated parameters: $\theta_i^{'}$
\end{algorithmic}
\end{algorithm}

\subsection{Meta-learning}
We employ meta-learning for our model training to guarantee that the initial parameters $\theta$ exhibit robust generalization capabilities, facilitating rapid online optimization. MAML++ \cite{antoniou2018train} is an ideal strategy for our purpose, as it is designed to learn suitable initial model parameters optimized for swift adaptation to new tasks. The complete algorithm is detailed in Algorithm \ref{meta-learning}.
\begin{algorithm}
\caption{SSM-SAM Offline Meta-learner}
\label{meta-learning}
\begin{algorithmic}[1] % '1' 表示每行都显示数字
\IState \textbf{Input:} organ set $O$; initial weight and learning rate $\theta,\beta$
\IState \textbf{Require:} number of epochs $E$; number of within organ optimization steps $S$; online learning rate $\alpha$
\For{$e$ from 1 to $E$}
    \State Sample $T$ organs $\{o_1,o_2,...,o_T\}$ from $O$
    \For{$i$ from 1 to $T$}
        \State $\theta_i^{'} \gets \theta$
        \State Sample $K$ image-mask pairs $P_{i}=\{(I_{i},M_{i})_k\}$ 
        \Statex \hspace{3em}of the target organ $o_i$
        \State $\theta_i^{'}\gets$\textbf{Online Optimizer}($S,P_i,\theta_i^{'},\alpha$)
        %\For{$s$ from 1 to $S$}
        %    \For{$(I_i,M_i)_k$ in $P_i$}
        %        \State Update parameters:
        %        \Statex \hspace{6em} $\theta_i^{'} \gets \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{O_i}(f_{\theta_i^{'}}((I_i,M_i)_k))$
        %    \EndFor
        %\EndFor
    \EndFor
    \State Resample $K$ images-mask pairs $P_{i}^{'}$ for each $o_i$
    \State $\beta \gets \textbf{CosineAnnealingLR}(\beta,e)$
    \State $\theta \gets \theta-\beta\nabla_{\theta}\frac{1}{T}\sum_i^{T}L_{o_i}(f_{\theta_i^{'}}(P_i^{'}))$
\EndFor
\IState \textbf{Output:} updated parameters: $\theta$
\end{algorithmic}
\end{algorithm}
Note that % the two innermost for-loops are the same as online optimization in Algorithm \ref{online}, and 
 the outermost for-loop is the meta-learner, which is defined as follows:
\begin{equation}
    \theta \gets \theta-\beta\nabla_{\theta}\frac{1}{T}\sum_i^{T}L_{o_i}(f_{\theta_i^{'}})
\end{equation}
where $i$ is the $i^{th}$ organ. $T$ is the number of organs in a task batch for optimizing the meta-learner. We incorporate the cosine annealing learning rate as recommended in \cite{antoniou2018train} to enhance our model's efficiency in fitting the training set. 



==> 4_Approach2.tex <==
\subsection{Adapted Image Encoder}
The image encoder of SAM uses a Vision Transformer (ViT) \cite{dosovitskiy2021image}, which is pre-trained with MAE \cite{he2022masked}. When given an image of any size, it is essential to first resize it to a resolution of 1024 x 1024. The ViT then processes this resized image to generate an image embedding with dimensions $C\times H\times W$. For this research, we chose the ViT-B variant (SAM-b), (where $C$ = 256, $H$ = 64, $W$ = 64).  To enable efficient learning with faster updates and address the issue of excessive GPU memory usage, we keep the image encoder frozen and inject a trainable \textbf{Adapter} to each of the 12 transformer layers as mentioned before. We only train the parameters within \textbf{Adapters}, which are tasked with learning task-specific knowledge and low-level structural information from the features extracted from image embeddings. For the $k$-$th$ Adapter layer, we take patch embedding $\text{F}^{k}$ as input and obtain updated parameters $\text{P}^{k}$
\begin{equation} 
\text{P}^{k} = \text{{MLP}}_{\text{{up}}}(\text{{GELU}}(\text{{MLP}}^{k}_{\text{{tune}}} (F^{k}))
\end{equation}
where $\text{{MLP}}^{k}_{\text{{tune}}}$ refers to a linear layer within each Adapter for generating distinct prompts. $\text{{MLP}}_{\text{{up}}}$ is an up-projection layer shared across all Adapters designed to match the dimension of transformer features. $\text{P}^{k}$ represents the output associated with each transformer layer. 

Also, we divided image encoder to four sub-blocks, which is carried out with the intent of deriving multi-level information \cite{li2022exploring}. After passing through the image encoder, these four image embeddings of size $B \times 256 \times 64 \times 64 $ are fed into the subsequent module.

% Also, we divided image encoder to four sub-blocks, which is carried out with the intent of deriving multi-level information \cite{li2022exploring}. After passing through the image encoder, there are four embeddings of size $B \times C \times H \times W $. We perform a self-sampling operation on the first image embedding to update it. Subsequently, these four features are individually input into the Flexible Mask Attention Module (FMAM) to form a feature of size $B \times 1024 \times 64 \times 64$. We then apply a series of convolution and upsampling to generate the predicted mask. Note that for fully supervised learning, we only remove the Flexible Mask Attention Module in the decoder, and all other parts remain the same. We use an online meta-learning-based optimizer for few-shot learning to fast adapt to unseen organs. 


% To avoid fine-tuning the whole large image encoder of SAM, we keep it in a frozen state and introduce a minimal amount of learnable parameters\cite{liu2023explicit}. We only train these parameters within adapters are tasked with learning task-specific knowledge and low-level structural information from the features extracted from image embeddings. 
% % This process can be summarized as 
% % \begin{equation}
% % \text{P}^{i} = \text{{MLP}}_{\text{{up}}}(\text{{GELU}}(\text{{MLP}}^{i}_{\text{{tune}}} (F_{\text{{pe}}} + F_{\text{{hf}}}))
% % \end{equation}


% For the image encoder component, we keep it in a frozen state and introduce a minimal amount of trainable parameters.
% The Adapters are aimed to avoid fine-tuning the whole large image encoder of SAM \cite{liu2023explicit}. We only train these parameters within adapters are tasked with learning task-specific knowledge and low-level structural information from the features extracted from image embeddings. 
 
% The architecture of the Adapters is depicted on the left side of \cref{fig:1}. In pursuit of simplicity and efficiency, we have designed the adapter to incorporate merely two MLPs, with an GELU \cite{hendrycks2016gaussian} activation function interspersed between them. Specifically, the adapter utilizes information about patch embeddings to acclimate to the new task and employs high-frequency information \cite{xie2021segformer} to refine low-level features.
% \begin{equation}
% \text{P}^{i} = \text{{MLP}}_{\text{{up}}}(\text{{GELU}}(\text{{MLP}}^{i}_{\text{{tune}}} (F_{\text{{pe}}} + F_{\text{{hf}}}))
% \end{equation}
% where $\text{{MLP}}^{i}_{\text{{tune}}}$ refers to a linear layer within each Adapter for generating distinct prompts. $\text{{MLP}}_{\text{{up}}}$ is an up-projection layer shared across all Adapters designed to match the dimension of transformer features.$\text{P}^{i}$ represents the output prompting associated with each transformer layer.

% % \subsection{Few-shot Online Optimizer}
% % Segmentation models' clinical deployment has historically been hindered by a mismatch in distributions between training and testing datasets. Given the impossibility of collecting comprehensive representative data, we've innovated in our training approach. Rather than creating a universal offline model, we designed our model to recognize and adapt to new data types, ensuring it remains relevant for unseen images. In our few-shot medical image segmentation scenario, we consider a distribution over organs, denoted as $p(O)$, to which we aim our model to adapt. We represent our model as $f_\theta$ with parameter $\theta$, and it's trained on images of different organs, $I_{o_i}$, following the distribution $p(I_{o_i})$, where $o_i$ signifies the $i^{th}$ organ. The online optimizer optimises the parameters via back-propagating steps as follows:
% % \begin{equation}
% %     \theta_i^{'} \leftarrow \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{o_i}(f_{\theta_i^{'}})
% % \end{equation}
% % where $\alpha$ is the learning rate and $\theta_i^{'}$ represents the model parameters adapted to fit the $i^{th}$ organ. Please see equation x for the definition of loss function $L_{o_i}$. The overview of the online optimizer is outlined in \cref{online}.

% % \begin{algorithm}
% % \caption{SSM-SAM Online Optimizer}
% % \label{online}
% % \begin{algorithmic}[1] % '1' 表示每行都显示数字
% % \IState \textbf{Input:} $K$ image-mask pairs $P_{i}=\{(I_{i},M_{i})_k\}$ of the target organ $o_i$
% % \IState \textbf{Input:} trained parameters: $\theta$
% % \IState \textbf{Require:} learning rate $\alpha$; number of online optimization steps $S$
% % \State $\theta_i^{'} \gets \theta$
% % \For{$s$ from 1 to $S$}
% %     \For{$(I^i,M^i)_k$ in $P^i$}
% %         \State Update parameters with gradient descent:
% %         \Statex \hspace{3em} $\theta_i^{'} \gets \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{O_i}(f_{\theta_i^{'}}((I^i,M^i)_k))$
% %     \EndFor
% % \EndFor
% % \IState \textbf{Output:} updated parameters: $\theta_i^{'}$
% % \end{algorithmic}
% % \end{algorithm}

% % \subsection{Meta-learning}
% % To guarantee that the initial parameters $\theta$ exhibit robust generalization capabilities, facilitating rapid online optimization, we employ meta-learning for our model training. MAML is an ideal strategy for our purpose, as it is designed to learn good initial model parameters optimized for swift adaptation to new tasks. The complete algorithm is detailed in Algorithm \ref{meta-learning}.
% % \begin{algorithm}
% % \caption{SSM-SAM Offline Meta-learner}
% % \label{meta-learning}
% % \begin{algorithmic}[1] % '1' 表示每行都显示数字
% % \IState \textbf{Input:} organ set $O$; initial weight and learning rate $\theta,\beta$
% % \IState \textbf{Require:} number of epochs $E$; number of within organ optimization steps $S$
% % \For{$e$ from 1 to $E$}
% %     \State Sample $T$ organs $\{o_1,o_2,...,o_T\}$ from $O$
% %     \For{$i$ from 1 to $T$}
% %         \State $\theta_i^{'} \gets \theta$
% %         \State Sample $K$ image-mask pairs $P_{i}=\{(I_{i},M_{i})_k\}$ 
% %         \Statex \hspace{3em}of the target organ $o_i$
% %         \For{$s$ from 1 to $S$}
% %             \For{$(I^i,M^i)_k$ in $P^i$}
% %                 \State Update parameters:
% %                 \Statex \hspace{6em} $\theta_i^{'} \gets \theta_i^{'}-\alpha\nabla_{\theta_i^{'}}L_{O_i}(f_{\theta_i^{'}}((I^i,M^i)_k))$
% %             \EndFor
% %         \EndFor
% %     \EndFor
% %     \State Resample $K$ images-mask pairs $P_{i}^{'}$ for each $o_i$
% %     \State $\beta \gets \textbf{CosineAnnealingLR}(\beta,e)$
% %     \State $\theta \gets \theta-\beta\nabla_{\theta}\frac{1}{T}\sum_i^{T}L_{o_i}(f_{\theta_i^{'}}(P_i^{'}))$
% % \EndFor
% % \IState \textbf{Output:} updated parameters: $\theta$
% % \end{algorithmic}
% % \end{algorithm}
% % Note that the two innermost for-loops are the same as online optimization in Algorithm \ref{online}, and The outermost for-loop is the meta-learner,which is defined as follows:
% % \begin{equation}
% %     \theta \gets \theta-\beta\nabla_{\theta}\frac{1}{T}\sum_i^{T}L_{o_i}(f_{\theta_i^{'}})
% % \end{equation}
% % Where $i$ is the $i^{th}$ organ. $T$ is the number of organs in a task batch for optimizing the meta-learner. To enhance our model's efficiency in fitting the training set, we incorporate the cosine annealing learning rate as recommended in \cite{antoniou2018train}. 

==> 4_Approach3.tex <==
\subsection{Self-Sampling Module}

\begin{figure}[ht!]
\centering
\includegraphics[height=6cm]{fig/self-sampling.pdf}
\caption{Structure of queries and prompt interaction during training and evaluation.}
\label{fig:2}
\end{figure}

\begin{figure*}[ht!]
\centering
\includegraphics[height=7.5cm]{fig/FMAM.pdf}
\caption{Process of Flexible Mask Attention Module (FMAM) and Flexible Mask Attention Decoder(FMAD).}
\label{FMAM}
\end{figure*}
We employ a \textit{positive-negative attention self-sampling} module inspired by \cite{zou2023segment} to convert all kinds of non-textual queries to visual prompts that lie in the same visual embedding space, as opposed to the conventional position encoding in SAM\cite{kirillov2023segment}. Our algorithm is illustrated in \cref{fig:2} and can be summarized as follows:
\begin{gather}
    P = \textbf{concatenate}([P_{postive}, P_{negative}]) \\
    P_{v} = \textbf{Self-Sampler} (P, Z_{h})
\end{gather}
where $P_{positive}$, $P_{negative}$ stand for positive points (region we aim to segment) and negative points (background region) sampled from the image, respectively. $Z_{h}$ is the feature maps extracted from the image and $P$ denotes the point prompts. 

Afterward, we concatenated these positive points and negative points to form the point prompts. This approach ensures that the model does not only focus on the positive parts, which could potentially lead to a higher false positive rate, but also adequately attends to the negative parts. With this method, the model can better discerns the organ boundaries, enhancing segmentation performance when we only give one point to prompt the model during inference.

On receiving the point prompts, we perform direct interpolation from the feature map to get the corresponding embeddings as visual prompts. This ensures that the prompts and the image embeddings share identical semantic features. We initialize a few tokens as learnable global queries and concatenate them with these visual prompts. After that, we apply self-attention \cite{vaswani2017attention} between a set of learnable queries and the visual prompts. Then, cross-attention is applied only between the image embeddings and these updated queries. 
 








==> 4_Approach4.tex <==
\subsection{Flexible Mask Attention Decoder}
Since we divided each 3D volume data into 12 chunks as in section \ref{setup}, there is a certain pattern to how each organ changes across different slices. This observation inspired us to treat the segmentation task like a tracking task. Consequently, we introduced the Flexible Mask Attention Decoder (FMAD). The core of this decoder is the Flexible Mask Attention Module (FMAM), as illustrated in Fig \ref{FMAM}. By leveraging cross-attention, we can expand or contract the blurred support mask to predict the mask for the query image, mitigating the challenge of direct mask prediction. The Gaussian blurred support masks provide the model with ample room to explore potential mask positions while efficiently suppressing distractions from other parts of the image. 

In decoding, the attention block bridges the Gaussian blurred support mask and queries images to update the mask. We first apply a Gaussian filter on original support mask $\textbf{M}\in\mathbb{R}^{H\times W\times 1}$, repeat it for $C$ times and reshape to $N\times C$ to get $\textbf{M}^{'}\in\mathbb{R}^{N\times C}$. Then we can easily cast it on query feature $\textbf{F}\in \mathbb{R}^{N\times C}$ extracted from image encoder to get $\textbf{K}\in \mathbb{R}^{N\times C}$ and $\textbf{Q}\in \mathbb{R}^{N\times C}$ as follows:
%\begin{gather}
%    \textbf{K}=(\textbf{M}^{'}\odot \textbf{F})\textbf{W}^{K} \\
%    \textbf{Q}=\textbf{F}\textbf{W}^{Q}
%\end{gather}
\begin{equation}
    \textbf{K}=(\textbf{M}^{'}\odot \textbf{F})\textbf{W}^{K} \\
\end{equation}

where $\odot$ means element-wise production, $\textbf{W}^{K}\in\mathbb{R}^{C\times C}$ means key projection matric. Following \cite{vaswani2017attention}, we also adopt the dot-product to compute the similarity matrix $\textbf{A}_{K\to Q}\in\mathbb{R}^{N\times C}$ between the query and key as follows:
\begin{equation}
    \textbf{A}_{K\to Q}=\mathrm{Atten}(\textbf{Q},\textbf{K})=\mathrm{Softmax_{col}}(\bar{\textbf{Q}}\bar{\textbf{K}}^{T}/\tau)
\end{equation}

where $\bar{\textbf{Q}}$ and $\bar{\textbf{K}}$ are $l_2$-normalized features of \textbf{Q} and \textbf{K} across the channel dimension, and $\tau$ is a temperature parameter controlling the Softmax distribution, which is the same as in \cite{wang2021transformer}. Then we convert $\textbf{M}^{'}$ to $\textbf{V}\in\mathbb{R}^{N\times C}$ though:
\begin{equation}
    \textbf{V}=(\textbf{M}^{'})\textbf{W}^{V}
\end{equation}

where $\textbf{W}^{V}\in\mathbb{R}^{C\times C}$ denotes value projection matrix. With the attention matrix $\textbf{A}_{K\to Q}$ from key to query, we can transform the value via $\textbf{A}_{K\to Q}\textbf{V}\in \mathbb{R}^{N\times C}$.

Unlike typical attention layers, at the first residual connection, we use \textit{multiply} \& \textit{Norm} instead of \textit{Add} \& \textit{Norm} to propagate query feature \textbf{F} as follows:
\begin{equation}
    \textbf{F}^{'}=\mathrm{InsNorm}(\textbf{A}_{K\to Q}\textbf{V}\odot\textbf{F})
\end{equation}
By using the updated Gaussian mask from the attention layer, we can further refine the predicted mask. After processing each of the four image embeddings, we upsample, concatenate, and put them through a convolutional layer. This approach facilitates improved information integration across layers to predict the final mask.

==> 5_Experiments.tex <==
\section{Experiments}

==> 5_Experiments1.tex <==
\subsection{Setup}
\label{setup}
\textbf{Datasets} To verify the generality and robustness of our approach, we perform experiments on two datasets, ABD-30 and ABD-MRI. We evaluate the complete few-shot segmentation framework (SSM-SAM) on both datasets, while the backbone (SS-SAM) is only assessed on ABD-30 to validate its efficiency.

- ABD-30 (from MICCAI15 Multi-Atlas Abdomen Labeling challenge\cite{MICCAI}) contains 30 cases with 3779 axial abdominal clinical CT images. 

- ABD-MRI (from Combined Healthy Abdominal Organ Segmentation (CHAOS) challenge \cite{kavur2021chaos} held in IEEE International Symposium on Biomedical Imaging (ISBI) 2019) contains 20 3D abdominal MRI scans with total four different labels.

%We further evaluate our backbone (SS-SAM) on the skin lesion segmentation challenge using the ISIC 2018 \cite{codella2019skin} dataset. We follow \cite{azad2019bi} for the experimental setup.

Liver, spleen and left and right kidney are used as semantic classes following previous settings \cite{tang2021recurrent, ding2023few, ouyang2020self}. Within each experiment, one organ is considered as unseen semantic class for testing while the rest are used for training.
% We use the training set released in the MICCAI 2015 Multi-Atlas Abdomen Labeling Challenge as the fully-labeled dataset \cite{landman2015miccai}, which contains 30 abdominal CT scans (ABD-30) with 3779 axial contrast-enhanced abdominal clinical CT images in total. For each case, 13 anatomical structures are annotated, including spleen, right kidney, left kidney, gallbladder, esophagus, liver, stomach, aorta, inferior vena cava (IVC), portal vein splenic vein, pancreas, left adrenal gland, right adrenal gland. Each CT volume consists of 85 $\sim$ 198 slices of 512 × 512 pixels, with a voxel spatial resolution of ([0.54 $\sim$ 0.54] × [0.98 $\sim$ 0.98] × [2.5 $\sim$ 5.0]) \SI{}{\cubic\milli\meter}.
% Following previous settings \cite{tang2021recurrent, ding2023few, ouyang2020self}, we only select four conjunct labels: left kidney, right kidney, liver, and spleen to evaluate our methods for both supervised learning and few-shot learning.

\textbf{Evaluation Metrics}  We use the Dice Similarity Coefficient (DSC) to evaluate the prediction mask \textbf{m} against the ground truth mask \textbf{g}:

\begin{equation}
    \text{{DSC(m, g)}} = \frac{2 \left | m\cap g \right |}{\left | m \right |  + \left |  g \right | }
\end{equation}

% \textbf{Loss function}
% We supervise our network using balanced cross entropy loss and iou loss between the predicted mask X and ground truth segmentation mask Y:
% \begin{gather}
%     L_{seg} = L_{bce} + L_{iou} \\
%     L_{bce} = -\frac{1}{HWC} \sum\limits_{h,w,c} [Y_{h,w,c} \cdot \log(\sigma(X_{h,w,c})) \nonumber \\
%     + (1 - Y_{h,w,c}) \cdot \log(1 - \sigma(X_{h,w,c}))] \\
%     L_{iou} = 1 - \frac{\sum\limits_{h,w} X_{h,w} \times Y_{h,w}} {\sum\limits_{h,w} (X_{h,w} + Y_{h,w}) - \sum\limits_{h,w} X_{h,w} \times Y_{h,w}}
% \end{gather}
% where $\sigma$ as the sigmoid function.

\textbf{Implementation Details}
All the images extracted from 3D volume data are reshaped to $1024\times1024$ to fit into the SAM model. We follow the same protocol used in \cite{tang2021recurrent,ouyang2020self,roy2020squeeze} to do 1-way 1-shot learning by dividing the 3D CT scans into 12 chunks and segmenting all the query slices in one chunk by using the center slice in the chunk as the support image, see Fig.\ref{fig:4} for visual representation.
\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\textwidth]{fig/chunk_illustrate.pdf}
\caption{Representative chunk}
\label{fig:4}
\end{figure}
We use ViT-B \cite{dosovitskiy2021image} version of SAM and supervise our network using balanced cross entropy loss and IoU loss as \cref{loss} between the predicted mask and ground truth mask. AdamW optimizer \cite{loshchilov2017decoupled} is used for all the experiments with an initial learning rate of 2e-4. Cosine decay\cite{antoniou2018train} is applied to the learning rate. Few-shot segmentation task is trained for 50 epochs on a single NVIDIA A40 GPU and fully supervised segmentation task is trained for 50 epochs using PyTorch on a single NVIDIA RTX 3090 GPU.

==> 5_Experiments2.tex <==
\subsection{Main Results}   
% \setlength{\abovecaptionskip}{10pt}
% \setlength{\belowcaptionskip}{5pt}

\begin{table*}[ht!]
\centering
\begin{tabular}{|c|c|cccc|c|}
\hline Dataset & Method & Spleen $\uparrow$ & Kidney L $\uparrow$ & Kidney R $\uparrow$ & Liver $\uparrow$ & mean $\uparrow$\\
\hline
 \multirow{9}{*}{ABD-30}& SE-Net \cite{roy2020squeeze} & 0.23 & 32.83 & 14.34 & 0.27 & 11.91 \\
 &PANet \cite{wang2019panet} & 25.59 & 32.34 & 17.37 & 38.42 & 29.42 \\
 &SSL-ALPNet \cite{ouyang2020self} & 60.25 & 63.34 & 54.82 & 73.65 & 63.02 \\
 &Affine & 48.99 & 43.44 & 45.67 & 68.93 & 51.75 \\
 &RP-Net \cite{tang2021recurrent} & 72.19 & 75.03 & 70.89 & 80.53 & 74.66 \\
 \cline{2-7}
 &\textbf{SS-SAM (w/o MAML++, w/o FMAD)} & 77.24 & 72.89 & 79.78 & 72.00 & 75.48\\
 &\textbf{SS-SAM (w/o MAML++, w/ FMAD)} & 78.99 & 73.33 & 83.49 & 74.81 & 77.65\\
 &\textbf{SSM-SAM (w/ MAML++, w/o FMAD)} & 80.55 & 77.83 & 82.79 & 82.70 & 81.46\\
 \cline{2-7}
 &\textbf{SSM-SAM (w/ MAML++, w/ FMAD)} & \textbf{86.95} & \textbf{80.96} & \textbf{84.47} & \textbf{87.12} & \textbf{84.87}\\
 \hline
 \hline
 \multirow{9}{*}{ABD-MRI}& SE-Net\cite{roy2020squeeze}& 51.80 & 62.11 & 61.32 & 27.43 & 50.66\\
 & PANet\cite{wang2019panet}& 50.90 & 53.45 & 38.64 & 42.26 & 46.33\\
 & SSL-ALPNet\cite{ouyang2020self}& 67.02 & 73.63 & 78.39 & 73.05 & 73.02\\
 & Affine & 62.87 & 64.70 & 69.10 & 65.00 & 65.41\\
 & RP-Net \cite{tang2021recurrent} & 75.69 & 79.30 & \textbf{84.66} & 71.51 & 77.79\\
 \cline{2-7}
 &\textbf{SS-SAM (w/o MAML++, w/o FMAD)} & 71.99 & 76.52 & 72.13 & 69.36 & 72.50 \\
 &\textbf{SS-SAM (w/o MAML++, w/ FMAD)} & 73.64 & 78.04 & 76.69 & 72.13 & 75.12\\
 &\textbf{SSM-SAM (w/ MAML++, w/o FMAD)} & 76.77 & 80.47 & 77.44 & 76.32 & 77.75\\
 \cline{2-7}
 & \textbf{SSM-SAM (w/ MAML++, w/ FMAD)} & \textbf{78.81} & \textbf{81.70} & 80.38 & \textbf{77.50} & \textbf{79.59}\\
 \hline
\end{tabular}
\smallskip
\caption{DSC comparison with other methods on ABD-30 and ABD-MRI for few-shot learning (unit:\%).}
\label{tab:few-shot}
\end{table*}

\begin{table*}[ht!]
\centering
\begin{tabular}{|c|c|cccccccc|}
\hline 
  Method & DSC $\uparrow$ & Aorta & Gallbladder& Kidney(L) & Kidney(R) & Liver & Pancreas & Spleen & Stomach \\
\hline
 TransUNet \cite{chen2021transunet} & 77.48 & 87.23 & 63.13 & 81.87 &  77.02 & 94.08 & 55.86 & 85.08 & 75.62\\
 SwinUnet \cite{cao2022swin} & 79.13 & 85.47 & 66.53 & 83.28 & 79.61 & 94.29 & 56.58 & 90.66 & 76.60\\
 MissFormer \cite{huang2022missformer} & 81.96 & 86.99 & 68.65 & 85.21 & 82.00 & 94.41 & 65.67 & 91.92 & 80.81\\
 % TransDeepLab \cite{azad2022transdeeplab} & 80.16 & 86.04 & 69.16 & 84.08 & 79.88 & 93.53 & 61.19 &  89.00 & 78.40\\
 HiFormer \cite{heidari2023hiformer} & 80.39 & 86.21 & 65.69 & 85.23 & 79.77 & 94.61 & 59.52 & 90.99 & 81.08\\
 DAE-Former \cite{azad2022dae} & 82.43 & 88.96 & 72.30 & 86.08 & 80.88 & 94.98 & 65.12 & 91.94 & 79.19 \\
 PaNN \cite{zhou2019prior} & 90.8 & 92.5 & 72.9 & 95.3 & 92.0 & 95.3 & - & \textbf{96.8} & - \\
 \hline
 \textit{\textcolor{blue}{MissFormer}} \cite{huang2022missformer} & 
 \textit{\textcolor{blue}{78.84}} & \textit{\textcolor{blue}{85.89}} & 
 \textit{\textcolor{blue}{64.75}} & \textit{\textcolor{blue}{84.19}} &
 \textit{\textcolor{blue}{76.98}} & \textit{\textcolor{blue}{94.18}} &
 \textit{\textcolor{blue}{55.19}} & \textit{\textcolor{blue}{89.07}} & \textit{\textcolor{blue}{80.47}} \\
 
 \textit{\textcolor{blue}{HiFormer}} \cite{heidari2023hiformer} & \textit{\textcolor{blue}{78.24}} & \textit{\textcolor{blue}{85.94}} & \textit{\textcolor{blue}{60.88}} & \textit{\textcolor{blue}{84.16}} & \textit{\textcolor{blue}{76.57}} & \textit{\textcolor{blue}{94.54}} & \textit{\textcolor{blue}{54.00}} & \textit{\textcolor{blue}{89.81}} & \textit{\textcolor{blue}{80.02}} \\

 \textit{\textcolor{blue}{DAE-Former}} \cite{azad2022dae} &
 \textit{\textcolor{blue}{80.46}} & \textit{\textcolor{blue}{87.26}} & 
 \textit{\textcolor{blue}{67.46}} & \textit{\textcolor{blue}{82.15}} & \textit{\textcolor{blue}{77.53}} & \textit{\textcolor{blue}{94.36}} & \textit{\textcolor{blue}{63.32}} & \textit{\textcolor{blue}{90.85}} & \textit{\textcolor{blue}{80.77}} \\
 \hline
 SAMed \cite{zhang2023customized} & 81.88 & 87.77 & 69.11 & 80.45 & 79.95 & 94.80 & 72.17 & 88.72 & 82.06\\
%  MedSAM \cite{ma2023segment} & 67.14 & 82.56 & 89.39 & 71.24 & 77.58 \\
 SAM Adapter \cite{chen2023sam} & 92.01 & 95.35 & 87.88 & \textbf{96.16} & 96.73 & 97.23 & \textbf{79.86} & 90.60 & 92.26 \\
\hline
%  %\hline SAM \cite{kirillov2023segment} & 63.20 & 77.01 & 75.93 & 57.72 & \\
 \textbf{SS-SAM} & \textbf{93.09} & \textbf{95.96} & \textbf{89.77} & 96.09 & \textbf{96.79} & \textbf{97.61} & 79.15 & 95.15 & \textbf{94.23}\\
\hline
\end{tabular}
\smallskip
\caption{Comparison to state-of-the-art models using a fully supervised method on the ABD-30 dataset. Best results are highlighted in bold (unit:\%). For a fair comparison, the results in italics are from the corresponding model with the same self-sampling module. Notably, our modified SAM (SS-SAM) outperforms other leading models.}
\label{tab:fully}
\end{table*}


\textbf{Results on Few-shot Medical Image Segmentation} Table \ref{tab:few-shot} shows the few-shot segmentation performance of SSM-SAM with previous work on ABD-30 and ABD-MRI respectively. SE-Net \cite{roy2020squeeze} represents the first architecture designed explicitly for few-shot medical image segmentation. PANet \cite{wang2019panet} is an extended version of the widely-used prototypical network \cite{snell2017prototypical}, tailored for natural image segmentation. SSL-ALPNet \cite{ouyang2020self} integrates self-supervised learning with prototypical networks. Affine denotes the accuracy result after aligning the support and query images globally using an affine transformation. RP-Net \cite{tang2021recurrent} stands as the state-of-the-art framework for few-shot medical image segmentation, leveraging both a context relation encoder and a recurrent module. \cite{tang2021recurrent} reported performance for all the methods above, so these numbers are directly quoted.

%From \cref{tab:few-shot}, it can be observed that on the CT and MRI datasets, the use of FMAD results in improvements of 2.17\% $\sim$ 3.41\% and 1.84\% $\sim$ 2.62\%. Additionally, employing the MAML++ based optimizer leads to enhancements of 5.98\% $\sim$ 7.22\% and 4.47\% $\sim$ 5.25\%, respectively. 

%This indicates that both our meta-optimizer and FMAD are highly effective. Our method outperforms state-of-the-art method by an average of 10.21\% and 1.80\% on ABD-30 and ABD-MRI, respectively.

First, compared to state-of-the-art method RP-Net, SSM-SAM outperforms RP-Net by 10.21\% and 1.80\% on ABD-30 and ABD-MRI respectively. Second, the use of FMAD results in improvements of 2.17\% $\sim$ 3.41\% and 1.84\% $\sim$ 2.62\% respectively. Additionally, employing the MAML++ based optimizer leads to enhancements of 5.98\% $\sim$ 7.22\% and 4.47\% $\sim$ 5.25\% respectively. This indicates that both our meta-optimizer and FMAD are highly effective.

\textbf{Results on Fully Supervised Medical Image Segmentation}


% \begin{table}[ht!]
% \centering
% \begin{tabular}{|c|cccc|}
% \hline 
%   Method & DSC $\uparrow$ & SE $\uparrow$ & SP$\uparrow$ & ACC $\uparrow$  \\
% \hline
%  SwinUnet \cite{cao2022swin} & 0.8946 &  0.9056 & 0.9798 & 0.9645 \\
%  HiFormer \cite{heidari2023hiformer} & \textbf{0.9102} & 0.9119 & 0.9755 & 0.9621 \\
%  \hline
%  \textit{\textcolor{blue}{HiFormer}} \cite{huang2022missformer} & \textit{\textcolor{blue}{0.8981}} & \textit{\textcolor{blue}{0.9143}} & \textit{\textcolor{blue}{0.9552}} & \textit{\textcolor{blue}{0.9393}} \\
%  \hline
%  SAM Adapter \cite{chen2023sam} & 0.8973 & 0.8920 & 0.9696 & 0.9452 \\
% \hline
%  %\hline SAM \cite{kirillov2023segment} & 63.20 & 77.01 & 75.93 & 57.72 & \\
%  \textbf{Ours} & 0.8991 & \textbf{0.9189} & \textbf{0.9810} & \textbf{0.9651} \\
% \hline
% \end{tabular}
% \smallskip
% \caption{Performance comparison of the proposed method against the SOTA approaches on the ISIC2018 skin lesion segmentation task.}
% \label{tab:skin}
% \end{table}
To evaluate the performance of our backbone (without MAML++), we compare SS-SAM with recent SOTA methods on ABD-30 dataset without Flexible Mask Attention Module, including U-Net \cite{ronneberger2015u}, Att-UNet \cite{oktay2018attention}, TransUnet \cite{chen2021transunet}, Swin-Unet \cite{cao2022swin}, MissFormer \cite{huang2022missformer}, TransDeepLab \cite{azad2022transdeeplab}, HiFormer \cite{heidari2023hiformer}, DAE-Former \cite{azad2022dae} and SAMed \cite{zhang2023customized} following \cite{zhang2023customized}. For a fair comparison, we integrate the self-sampling module into some of the state-of-the-art models because the original SAM and our method utilize visual prompts, which incorporate ground truth information into the model while previous state-of-the-art models did not leverage such additional information. The results are highlighted in blue italics in \cref{tab:fully}. Surprisingly, since these models are unaware of how to process this information, their performance slightly declined. We also observe that SS-SAM achieves state-of-the-art performance. These experiments demonstrate that our models are capable of achieving high performance and also refute the potential claim that introducing prompts is a form of "cheating".

% The performance metrics for PANet-init, PANet, SE-Net, and SSL-ALPNet on ABD-30 and ABD-MRI were reported by \cite{tang2021recurrent}, so these figures are directly quoted. 
%In contrast, previous state-of-the-art models did not leverage such additional information.
% \textbf{Results on Skin Lesion Segmentation} The comparison results for benchmarks of ISIC 2018 skin lesion segmentation task against leading methods are presented in \cref{tab:skin}. It can be observed that, compared to both CNN and Transformer-based methods, our network achieves superior performance across almost all metrics. Note: Similar to \cref{tab:fully}, for a fair comparison, models that incorporate prompts with ground truth information are denoted in blue italics. As seen with Synapse dataset, when models are unaware of how to process this information, their performance slightly deteriorates. This once again indicates that a traditional model + prompt doesn't necessarily outperform a universal foundation model. It also refutes the potential claim that introducing prompts is a form of "cheating".


% Second, although there are no special network structure designed for a certain task, we still beat the SOTA for each of the two tasks. Furthermore, our model exhibited improvements over the SAM that only employs the Adapter.



==> 5_Experiments3.tex <==
\subsection{Ablation Study}  

\begin{table*}[ht!]%bp]
\centering
\begin{tabular}{|c|cccc|c|}
\hline 
Prompt & Spleen & Kidney L & Kidney R & Liver & Mean \\
\hline
 no prompt & 91.83 & 93.65 &  92.55 & 96.21 & 93.56 \\
 w/ position encoding & 93.05 & 95.75 & \textbf{96.87} & 97.27 & 95.74 \\
w/ self-sampling & \textbf{95.15} & \textbf{96.09} & 96.79 & \textbf{97.61} & \textbf{96.41}  \\
\hline
\end{tabular}
\smallskip
\caption{Ablation Study on no prompt, position encoding (pe) of points and self-sampling}
\label{tab:3}
\end{table*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=0.89\textwidth]{fig/ablation_meta.pdf}
\caption{Testing process of MAML++ based model (in deep blue) and  Fine-tuning of a model pretrained on the same distribution of tasks without MAML++ (in light blue)}
\label{fig:5}
\end{figure*}

% \begin{table*}[ht!]
% \centering
% \begin{tabular}{|c|c|cccc|c|}
% \hline Dataset & Method & Spleen $\uparrow$ & Kidney L $\uparrow$ & Kidney R $\uparrow$ & Liver $\uparrow$ & mean $\uparrow$\\
% \hline
%  \multirow{4}{*}{ABD-30}
%  %\cline{2-7}
%  &\textbf{SS-SAM (w/o MAML++, w/o FMAD)} & 77.24 & 72.89 & 79.78 & 72.00 & 75.48\\
%  &\textbf{SS-SAM (w/o MAML++, w/ FMAD)} & 78.99 & 73.33 & 83.49 & 74.81 & 77.65\\
%  &\textbf{SSM-SAM (w/ MAML++, w/o FMAD)} & 80.55 & 77.83 & 82.79 & 82.70 & 81.46\\
%  \cline{2-7}
%  &\textbf{SSM-SAM (w/ MAML++, w/ FMAD)} & \textbf{86.95} & \textbf{80.96} & \textbf{84.47} & \textbf{87.12} & \textbf{84.87}\\
%  \hline
%  \hline
%  \multirow{4}{*}{ABD-MRI}
%  %\cline{2-7}
%  &\textbf{SS-SAM (w/o MAML++, w/o FMAD)} & 71.99 & 76.52 & 72.13 & 69.36 & 72.50 \\
%  &\textbf{SS-SAM (w/o MAML++, w/ FMAD)} & 73.64 & 78.04 & 76.69 & 72.13 & 75.12\\
%  &\textbf{SSM-SAM (w/ MAML++, w/o FMAD)} & 76.77 & 80.47 & 77.44 & 76.32 & 77.75\\
%  \cline{2-7}
%  & \textbf{SSM-SAM (w/ MAML++, w/ FMAD)} & \textbf{78.81} & \textbf{81.70} & 80.38 & \textbf{77.50} & \textbf{79.59}\\
%  \hline
% \end{tabular}
% \smallskip
% \caption{DSC comparison with other methods on ABD-30 and ABD-MRI for few-shot learning (unit:\%).}
% \label{tab:few-shot-ablation}
% \end{table*}

% \begin{table*}[ht!]
% \centering
% \begin{tabular}{|c|cccc|c|}
% \hline 
%  Decoder & Spleen $\uparrow$ & Kidney L $\uparrow$ & Kidney R $\uparrow$ & Liver $\uparrow$ & mean $\uparrow$\\
% \hline
%  Mask Decoder & 84.72 & 85.94 & 80.46 & 86.49 & 84.40 \\
%  IUD  & 92.07 & 93.60 & 96.52 & 97.41 & 94.90\\
%  SUD  & \textbf{95.15} & \textbf{96.09} & \textbf{96.79} & \textbf{97.61} & \textbf{96.41}  \\
% \hline
% \end{tabular}
% \smallskip
% \caption{Ablation Study on a) original Mask Decoder of SAM, b) Iterative Upsampling Decoder (IUD) and c) Single Upsampling Decoder (SUD)}
% \label{tab:4}
% \end{table*}

\textbf{Effect of self-sampling.} As previously explained, the self-sampling module derives visual prompts by interpolating between the provided point coordinates and image embeddings. Subsequently, it conducts cross-attention with the image embeddings. On the other hand, SAM's point prompt employs positional encoding on the points before performing cross-attention with the image embeddings. These two approaches differ in their treatment of the sampled points. To evaluate the effectiveness of the proposed methods, we performed ablation studies on four distinct organs: the spleen, left kidney, right kidney, and liver, using a fully supervised approach. For each organ, we kept the image encoder and decoder the same, with three different prompt methods: a) no prompt, b) point prompt with position encoding, and c) point prompt with self-sampling. As presented in \cref{tab:3}, our self-sampling method achieved the highest mean DSC.

% \textbf{Effects of Iterative Upsampling.} We experimented with two distinct decoders: the Single Upsampling Decoder (SUD), which directly upsamples the mask map generated from concatenated image embeddings using a single convolutional operation, and the Iterative Upsampling Decoder (IUD), which alternates between convolution layers and upsampling operations four times. As mentioned in Section 3.4, our experiments demonstrate that iterative convolutional upsampling outperforms both the shallow attention layer approach and the method of directly generating a mask after multi-level aggregation from \cref{tab:4}. A potential rationale for the suboptimal performance of SUD may be that the feature outputs from various transformer layers lack the advantages inherent to the resolution pyramid observed in the Feature Pyramid Network (FPN). In the case of the mask decoder, a plausible explanation is that, even the absence of pyramid features, the convolution layers are capable to recover low-level information through the iterative refinement of the generated mask maps.



\textbf{Effects of Meta-learner.} To highlight the few-shot learning advantages of our model achieved by integrating a meta-learner, apart from the experiment setting in \cref{tab:few-shot}, we set up a more rigorous experimental setting to compare performances with and without the meta-learner.

Following the configurations specified in \cite{finn2017model, li2020fss}, we selected only 125 images for the four organs. In each experiment, one organ is chosen as the test task (e.g., liver), while the remaining three organs (spleen, left kidney, right kidney) are used as training tasks. Only five images of each training task (spleen, left kidney, right kidney) are allocated during training. During testing, we adopt a 1-way, 5-shot approach, using five images of the test task (liver) as the support set for training. The remaining 120 images serve as the query set to evaluate the model's performance. 
%\cref{fig:5} displays the performance of models pre-trained and meta-trained using the same data across different epochs during the testing phase.

% In line with the configurations specified in \cite{finn2017model, li2020fss}, each organ is represented by five images in the training set. For the performance evaluation, we designated a set of 125 images for each organ. Contrary to the earlier approach, where CT scans were segmented into 12 different chunks, we randomly sampled the five training images from the support set. In our experimental setup, one organ is excluded and served as the test task during each training iteration. For clarity and consistency, we chose the spleen, left kidney, right kidney, and liver as the test tasks, echoing the selections made in section \ref{setup}.

Our findings were illuminating. A visual representation of the online optimization process of each of the four organs is provided in Fig.\ref{fig:5}. With just a limited number of training images, models equipped with the meta-learner outperformed those without by a significant margin of 12.07\% on average. Furthermore, models augmented by the meta-learner not only demonstrated swifter convergence in the initial epochs but also exhibited enhanced stability and performance in the concluding epochs. %This suggests that even in situations with scarce data, a minimal collection of images can be leveraged to achieve superior segmentation outcomes when using a model trained with the meta-learner. 

==> 5_Experiments4.tex <==
\subsection{Qualitative Results}
In Fig.\ref{result}, we present masks produced by SAM and variants of our algorithm. Notably, SAM struggles to segment smaller organs or those with indistinct boundaries. Conversely, SSM-SAM with FMAM outperforms its counterpart without FMAM, effectively minimizing the impact of similar distracting regions in the CT scans.

\begin{figure}[ht!]
\centering
\includegraphics[width=0.45\textwidth]{fig/results.pdf}
\caption{Examples of predictions of SAM, SSM-SAM without FMAM and SSM-SAM with FMAM}
\label{result}
\end{figure}

% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.7\textwidth]{fig/Qualitative_shadow.pdf}
% \caption{Qualitative Results of of different approaches on Shadow Detection. As illustrated in the figure, the SAM failed to distinguish the shadow and the background object. The SAM is used with the box prompt with the size of whole shadow as the input. Furthermore, it can be observed that the SAM Adapter produces some masks with both False Positives and False Negatives, while our framework does not exhibit this issue.}
% \label{fig:5}
% \end{figure*}

% To provide a more tangible understanding of our method's performance, we present qualitative results on several test samples. Fig \ref{fig:5} showcases the comparative visual outcomes generated by original SAM with box prompt, the baseline SAM Adapter method with point prompt, our framework, and the ground truth annotations.

% From the presented results, it is evident that our approach manages to capture intricate details and patterns that the baseline tends to overlook. Specifically, The original SAM struggles to accurately distinguish between shadowed and non-shadowed regions. The SAM Adapter often exhibits both False Positives (mistakenly classifying non-shadowed areas as shadowed shown in the fifth row and sixth row) and False Negatives (misidentifying shadowed regions as non-shadowed shown in the fourth row). Thanks to our proposed mechanism, our approach demonstrates enhanced stability and superior generalization capabilities.
% Furthermore, while the adapter method exhibits certain artifacts and noise, especially in regions with subtle color differences, our model produces cleaner and more coherent segmentations (as shown in the first, second and third row).

% These visual outcomes underscore the effectiveness of our proposed method, not only in terms of quantitative metrics, as discussed in the previous section, but also in the quality of segmentations it produces in real-world scenarios.




==> 6_Conclusions.tex <==
\section{Conclusions}
In this paper, we introduce a universal approach, SSM-SAM, designed to optimize and adapt a foundational model such as the Segment Anything Model (SAM), for few-shot medical image segmentation. Our method incorporates a positive-negative Self-Sampling prompt encoder and a Flexible Mask Attention Decoder to enhance the contextual relationship and tiny boundary information essential for mask generation. Moreover, our fast online meta-learning based optimizer facilitates high performance even without extensive training data and can be plugged into other frameworks effortlessly. Experiments demonstrate that SSM-SAM outperforms the previous state-of-the-art approach by as much as 10\% in terms of DSC. Furthermore, the proposed SSM-SAM can produce segmentations in just 50 seconds per organ, indicating its potential for real-time applications in medical settings.

